Leveraging Hierarchical Feature Sharing for Efficient Dataset Condensation

Given a real-world dataset, data condensation (DC) aims to synthesize a small synthetic dataset that captures the knowledge of a natural dataset while being usable for training models with comparable accuracy. Recent works propose to enhance DC with data parameterization, which condenses data into very compact parameterized data containers instead of images. The intuition behind data parameterization is to encode shared features of images to avoid additional storage costs. In this paper, we recognize that images share common features in a hierarchical way due to the inherent hierarchical structure of the classification system, which is overlooked by current data parameterization methods. To better align DC with this hierarchical nature and encourage more efficient information sharing inside data containers, we propose a novel data parameterization architecture, Hierarchical Memory Network (HMN). HMN stores condensed data in a three-tier structure, representing the dataset-level, class-level, and instance-level features. Another helpful property of the hierarchical architecture is that HMN naturally ensures good independence among images despite achieving information sharing. This enables instance-level pruning for HMN to reduce redundant information, thereby further minimizing redundancy and enhancing performance. We evaluate HMN on five public datasets and show that our proposed method outperforms all baselines.

==> tex/01_introduction-old.tex <==
\section{Introduction}

%(1) Define data condensation problem, introducing the term "memory budget". (2)  Currently, there are two orthogonal techniques. Say something about pros and cons and how far they are able to condense data. Synthetic data set versus a coreset selection (natural subset). For CIFAR-10, for 5 image per class, using synthetic data set 


%Data condensation methods, which use synthetic datasets, significantly outperform in terms of accuracy  another class of methods called coreset selection that select a subset of the dataset $D$ 

%Data distillation, also known as data condensation, is a technique introduced by Wang et al.~\cite{wang2018dataset} with the goal of this method is to create a smaller, synthesized dataset that effectively represents the original, larger training dataset. 

\ap{Insert cites}

Wang et al.~\cite{wang2018dataset} proposed {\em data condensation} (also called data distillation) as a technique to reduce the size of datasets required for training a given model.  Given a  dataset $D$, data condensation {\em synthesizes} a much smaller dataset $S$ that trains the model to achieve comparable performance to one trained with $D$. Data distillation offers advantages storage efficiency, training efficiency, as well as in continual learning domains where retaining and reusing representative samples for  retraining efficiently is important. The data distillation proposed by Wang required significantly fewer data points than another technique called coreset selection~\cite{coleman2019selection, toneva2018empirical, pleiss2020identifying, xiamoderate, zheng2022coverage} that uses a subset of data points of $D$.  More recent work has proposed a technique called {\em data parameterization} in which one synthesizes a  parameterized model $P$ (also called a {\em parameterized data container}) that can generate the entire synthetic dataset $S$, with $P$ requiring a smaller memory budget to store than $S$. \ap{Check following sentence: Also, perhaps say something on memory effiiciency of P versus S.} For instance, with CIFAR10 with ConvNet architecture, a parameterized model that generates only 1\% images compared to original dataset size can achieve 71\% model accuracy.  In this paper, we show that a parameterized model $P$ can be further optimized with respect to memory efficiency that state of the art techniques while achieving same or higher level of final accuracy of the model.





%is a technique introduced by Wang et al.~\cite{wang2018dataset} that aims to learn a small synthetic dataset $S$ that fits within a given memory budget that gives comparable accuracy in training models as the original, much larger dataset $D$. 



%By doing so, models can be trained on the condensed dataset and still achieve similar test performance as those trained on the entire training dataset. 
%Data condensation benefits a series of downstream applications such as continual learning~\cite{rosasco2022distilled, sangermano2022sample}, network architecture search~\cite{zhao2023dm}, and federated learning\cite{zhou2020distilled, song2022federated, xiong2022feddm}.
%Because of the considerable practical utility of data condensation, substantial efforts~\cite{zhao2021dataset, cazenavette2022dataset, zhao2023dm, dengremember, zhao2021dataset2} have been invested in improving its efficacy.
%DC~\cite{zhao2021dataset} generates condensed datasets by minimizing gradient distance between a batch of condensed data and a batch of real data. MTT~\cite{cazenavette2022dataset} seeks to match the training trajectories of models trained on the original dataset and the condensed dataset.
%Besides enhancing data condensation with better training loss, recent research~\cite{liudataset, kim2022dataset, dengremember} shows that \emph{data parameterization},  which condenses data into more advanced data containers rather than independent images, significantly improves data condensation performance. 
% IDC~\cite{kim2022dataset} store multiple images in a single image by down-sampling the condensed images.
%For instance, HaBa~\cite{liudataset} and LinBa~\cite{dengremember} concurrently propose factorization-based data parameterization approaches to encourage data sharing between different condensed images.

% DM~\cite{zhao2023dm} employs the maximum mean discrepancy on latent space between clean condensed data and real data across various random encoders to encourage condensed data to have a similar distribution to the original dataset. 
% \hz{What is the problem for the current methods? What is the major difference? We explore another potential way to design data container?}

% Although the SOTA data parameterization methods achieve promising performance improvement on the 

%In addition to data condensation, coreset selection~\cite{coleman2019selection, toneva2018empirical, pleiss2020identifying, xiamoderate, zheng2022coverage} is another orthogonal approach to augmenting data efficiency in the realm of deep learning. 
% Rather than generating a new dataset, coreset selection focuses on selecting a representative subset from the existing dataset. 
%Coreset selection improves data efficiency by discarding data points that contribute minimal information or, in certain instances, may even prove detrimental.
%Coreset selection is a potential way to enhance data condensation, given that condensed data can also have redundancy across different training images~\cite{liudataset}.
%However, the direct combination of coreset selection with data condensation is not straightforward. In contrast to the original training dataset, where each instance is independent, training examples generated by data containers, such as HaBa, can be interdependent due to shared parameters within the data containers. This interdependence complicates the application of coreset selection methods for pruning data containers, rendering it a non-trivial task.

Our key insight that data points from the same class can share class-level common information, and data points from different classes can share dataset-level common information. Based on this insight, we show that  parameterized models  of state-of-the-art methods can be further optimized with respect to memory efficiency by considering this potential common information across classes and within classes. But, leveraging this insight is non-trivial for recently-proposed data-parameterization methods since pruning any component of the model $P$ negatively can impact a broad set of generated examples $S$.

The main contribution of this paper is to show how to achieve that by proposing a novel dataset parameterization architecture called {\em Hierarchical Memory Network (HMN)} and then introduce a method for pruning redundant and detrimental  components from an HMN.  As illustrated in Figure~\ref{fig:HMN}, an HMN comprises a three-tier memory structure: general memory, class-level memory, and instance-level memory~~\footnote{It is important to note that, in contrast to classical generative models, HMN does not have any input, and the output of HMN is a fixed condensed synthetic dataset.}
Examples generated by HMNs share information via common general and class-level memory. 
Nevertheless, each generated example retains a degree of independence, as it utilizes a unique instance-level memory.

To achieve data efficiencies in the HMN, we show that ideas from earlier coreset selection techniques can be applied to instance memory in the HMN. \ap{This line is not clear.} Given a memory budget, we first condense an over-budget HMN (e.g., 10\% more size budget). Subsequently, we identify examples containing redundant or detrimental information and prune the corresponding instance-level memory for those examples.

We evaluate the efficacy of our proposed method by examining HMNs on three distinct image classification datasets: SVHN, CIFAR10, and CIFAR100. 
To enhance efficiency and scalability in data condensation, we utilize gradient matching~\cite{kim2022dataset, zhao2021dataset}, a low GPU memory consumption, batch-based loss technique, to condense information into HMNs. Remarkably, even when trained with this low-memory consumption batch-based loss, HMNs still surpass state-of-the-art (SOTA) methods.
For instance, we achieve $76.9\%$ accuracy on CIFAR10 using a storage budget of 50 images per class, which is $5.3\%$ higher than low-memory consumption SOTA methods and $3.3\%$ higher than all other SOTA methods. 
Large GPU memory consumption is still an open question in the area of data condensation. 
Our findings establish that, with an appropriate data parameterization method, the low-memory consumption batch-based loss can yield satisfactory performance, serving as a strong baseline for future studies on data condensation.

To summarize, our contributions are as follows:

\begin{enumerate}
\item  We propose a novel data parameterization model called Hierarchical Memory Network (HMN) for efficient data distillation. 
HMNs ensure better independence between different generated data points, which permits the pruning of individual examples that contribute less or negatively to final model accuracy.  
\item We propose a novel algorithm to prune the redundant or harmful information in an HMN. As far as we know, our work is the first paper to apply coreset selection on parametrized data containers for data condensation.

\item We evaluate the performance of HMNs on three image classification benchmarks and show that HMNs outperform all other baselines, even when we train HMNs with gradient matching, a low-memory consumption batch-based loss.

% \item  We propose a novel data parameterization method, Hierarchical Memory Network (HMN). HMNs ensure better independence between different generated images, which permits the pruning of individual examples.

% \item We also into a novel algorithm to prune the redundant or harmful information in HMN. As far as we know, our work is the first paper to apply coreset selection on data containers for data condensation.

\end{enumerate}


==> tex/99_checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerTODO{}
  \item Did you describe the limitations of your work?
    \answerTODO{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerTODO{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerTODO{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerTODO{}
        \item Did you include complete proofs of all theoretical results?
    \answerTODO{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerTODO{}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerTODO{}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerTODO{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerTODO{}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerTODO{}
  \item Did you mention the license of the assets?
    \answerTODO{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerTODO{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerTODO{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerTODO{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerTODO{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerTODO{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerTODO{}
\end{enumerate}


\end{enumerate}

==> tex/r1_rebuttal.tex <==

\newpage

% \twocolumn[{
% \begin{center}
% \captionsetup{type=table}
% \begin{tabular}{c|cccccccc}
%         \hline
%         IPC &  DC & DSA & DM & MTT & IDC & HaBa & LinBa & HMN (Ours)\\
%         \hline
%           1 & 4.6 & 6.6 & 3.9 & 8.8 & - & - & 16 & \textbf{19.3} \\
%           10 & 11.2 & 14.4 & 12.9 & 23.2 & - & - & - & \textbf{24.4} \\
%         \hline
%     \end{tabular}
% \captionof{table}{Accuracy (\%) performance comparison on Tiny ImageNet dataset. The evaluation results show that our proposed method achieves a better performance than all other baselines.}
% % \label{fig:semantic_pool}
% \end{center}

% \begin{center}
% \captionsetup{type=table}
% \begin{tabular}{c|ccc|ccc|ccc}
%         \hline
%         IPC &  \multicolumn{3}{c|}{1} &\multicolumn{3}{c|}{10} & \multicolumn{3}{c}{50}\\
%         \hline
%         Method &  HMN & IDC & HaBa & HMN & IDC & HaBa & HMN & IDC & HaBa\\
%         \hline
%         ConvNet &  \textbf{65.7} & 49.2 & 48.3 & \textbf{73.7} & 64.8 & 69.9 & \textbf{76.9} & 73.1 & 74\\
%         VGG16 &  \textbf{58.5} & 28.7 & 34.1 & \textbf{64.3} & 43.1 & 53.8 & \textbf{70.2} & 57.9 & 61.1 \\
%         ResNet18 &  \textbf{56.8} & 32.3 & 36.0 & \textbf{62.9} & 45.1 & 49.0 & \textbf{69.1} & 58.4 & 60.4\\
%         DenseNet121 &  \textbf{50.7} & 24.3 & 34.6 & \textbf{56.9} & 38.5 & 49.3 & \textbf{65.1} & 50.5 & 57.8\\
%         \hline
%     \end{tabular}
% \captionof{table}{ Transferability (accuracy \%) comparison to different model architectures. Due to the extremely long training time, we cannot reproduce the results on LinBa. Compared with IDC and HaBa, we find that HMN achieves better performance for all model architectures.}
% \end{center}
% }]

% \begin{table}
%     \centering
%     \begin{tabular}{c | c | c c c}
%         \hline
%         Data Container &  Loss & 1 IPC & 10 IPC & 50 IPC\\
%         \hline
%         Image & GM-IDC & 36.7 & 58.3 & 69.5 \\
%         IDC  & GM-IDC & 50 & 67.5 & 74.5 \\
%         HaBa & GM-IDC & 48.5 & 61.8 & 72.43 \\
%         LinBa & GM-IDC & 62.01 & 67.82 & 70.66 \\
%         HMN (Ours) & GM-IDC & \textbf{65.72} & \textbf{73.7} & \textbf{76.9} \\
%         \hline
%     \end{tabular}
%     \caption{Accuracy~(\%) performance comparison to data containers with the same training loss on CIFAR10. GM-IDC is the modified version of gradient matching loss used in the IDC paper.
%     The evaluation results find that HMN outperform all other data parameterization methods by a substantial margin.}
%     % \label{tab:my_label}
% \end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{c | c | c c c}
%         \hline
%         IPC &  Method & Loss & Acc. & Memory\\
%         \hline
%             \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}
%             1
%             % Loss Function
%             \end{tabular}} 
%         & HaBa & MTT & 48.3 & 3368M \\
%         & LinBa & BPTT & \textbf{66.4} & OOM \\
%          & HMN (Ours) & GM-IDC & 65.7 & \textbf{2680M} \\
%         \hline
%             \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}
%             10
%             % Loss Function
%             \end{tabular}} 
%           & HaBa & MTT & 69.9 & 11148M \\
%         & LinBa & BPTT & 71.2 & OOM \\
%          & HMN (Ours) & GM-IDC & \textbf{73.7} & \textbf{4540M} \\
%         \hline
%             \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}
%             50
%             % Loss Function
%             \end{tabular}} 
%           & HaBa & MTT & 74 & 48276M \\
%           & LinBa & BPTT & 73.6 & OOM \\
%           & HMN (Ours) & GM-IDC & \textbf{76.9} & \textbf{10426M} \\
%         \hline
%     \end{tabular}
%     \caption{Performance and memory comparison between LinBa, HaBa, and HMN trained with suggested loss in the corresponding papers on CIFAR10. We find that HMN achieves better or comparable performance compared to HaBa and LinBa. Specifically, LinBa is trained with BPTT with a very long trajectory, which leads to extremely large GPU memory consumption. LinBa official implementation offloads the GPU memory to CPU memory to address this issue. However, the context switch in memory offloading causes the training time to be intolerable. For example, LinBa needs about 14 days to condense a CIFAR10 1IPC dataset with a 2080TI, but using HMN with gradient matching only needs 15 hours to complete training on a 2080TI GPU.}
% \end{table}


